ML$^2$Tuner: Efficient Code Tuning via Multi-Level Machine Learning Models

The increasing complexity of deep learning models necessitates specialized hardware and software optimizations, particularly for deep learning accelerators. Existing autotuning methods often suffer from prolonged tuning times due to profiling invalid configurations, which can cause runtime errors. We introduce ML$^2$Tuner, a multi-level machine learning tuning technique that enhances autotuning efficiency by incorporating a validity prediction model to filter out invalid configurations and an advanced performance prediction model utilizing hidden features from the compilation process. Experimental results on an extended VTA accelerator demonstrate that ML$^2$Tuner achieves equivalent performance improvements using only 12.3% of the samples required with a similar approach as TVM and reduces invalid profiling attempts by an average of 60.8%, Highlighting its potential to enhance autotuning performance by filtering out invalid configurations

==> Paper/05_Algorithm.tex <==

\section{Methodology}

% \textbf{Training-stage} 
% \subsection{Tuning Cost}
% Get feature importance for general XGBoost Regression model without online learning.
% We trained on the full data and tested 20\% of the data.
% 어떻게 코스트를 탐색하고 최적화하는가?
% 학습을 진행하기 위해서는 먼저 search space에 대한 하이퍼파라미터 튜닝이 필요하다. 이는 grid search로 진행하였다. 
% 라이브러리에서 특수한 데이터들을 입력으로 주어 학습을 하기 때문에 일부 결과가 나오지 않는 경우들이 있다. 
% (결과를 표로 삽입하기)

템플릿 기반의 최적화 

제안된 방법론은 \predictParameter, \predictValidation 그리고 \predictLatency의 세 가지 단계를 포함하는 과정이다. 


본 섹션에서는 연구의 방향성과 기존 연구와 비교하였을 때 어떤 차이점와 기여점이 무엇인지 식별하고, 연구 진행 방향성에 대하여 소개한다. 기존 딥 러닝 컴파일러는 일반적인 auto-tuning에 사용되는 feature는 loop structure information (e.g., memory access count and data reuse ratio) 와 generic annotations (e.g., vectorization, unrolling, thread binding)을 활용하여 최적의 하이퍼 파라미터를 탐색한다. 실제 하드웨어에서 프로파일링의 횟수를 가능한 최소화하여 전반적인 신경망 모델의 프로파일링의 시간과 탐색 횟수를 단축시키는 목적으로 연구를 하였다.

기존 딥 러닝 컴파일러가 생성한 코드를 분석하는 과정에서 크게 2가지의 의문을 제기하게 되었다. (1) 컴파일러를 통해 생성된 코드의 문법적으로는 정상이라하더라도, 실제 하드웨어에서는 연산이 되지 않는 문제가 존재하였다. (2) 컴파일러로 부터 생성된 코드를 통해서 새로운 Feature를 추출하여, 새로운 의존성이 존재하는 Feature를 추출할 수 있다. 

% 본 연구에서는 2개의 변화점이 존재한다. 첫번째로는 신경망 모델의 레이어에 대한 하이퍼 파라미터의 값이 타겟 하드웨어에 대하여 유효한지 검증하는 Classification한 모델을 추가하였다. 두번째 변화로는 생성된 코드에 대하여 내부 Feature를 추출하여 추가적인 Hyper Parameter를 Exploit하여 더 빠른 시간에 수렴하는 `Cost Model`을 추가하였다.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=1\columnwidth]{Paper/Resources/3Stage_v2.png}
  \caption{\systemName의 전반적인 흐름도 (그림 이해에 최대한 이해가 되도록 돕는 내용)}
  \label{fig:nes_tuner_overview}
\end{figure*}

\subsection{Flow}

\systemName의 전반적인 구성은 2개의 Cost 모델과 유효 검증 모델, 컴파일 된 코드로 부터 Feature를 추출하는 Extractor로 구성이 되어 있다. Cost 모델은 (a)와 (f)에 있으며, (a)는 레이어의 구성 정보와 커널 구성 특징을 예측 성능 모델을 통해 Latency가 가장 낮을 것으로 예측되는 파라미터를 탐색 합니다. (f)는 Validation한 값들에 대하여 예상되는 성능치를 예상합니다. 유효한 Hyper Parameter의 값 만을 학습하도록 하고, 값의 성능을 예측하여 실제 하드웨어에서 연산을 하여 프로파일링 합니다. (c)는 새로운 데이터가 들어왔을 때 그 데이터가 유효한지, 즉 모델에 도움이 되는지를 평가하는 데 사용된다. 새로운 데이터를 평가하여 기준에 맞는 데이터만 학습 데이터에 추가되도록 한다.

초기의 검증은 무작위성을 지닌 Feature를 (a)에서 생성하고, (c) 또한 초기에는 부정확한 검증을 수행하여 총 20개의 Feature를 선택합니다. 그리고 코드를 생성한 뒤에 (e)를 통해 컴파일 된 코드에 대하여 Hidden Feature를 추출 합니다. 추출된 Hidden Feature과 함께 (a)에서 생성된 Feature과 함께 Latency 예측 모델 (f)를 통해 성능 예측을 수행합니다. 20개의 Feature에 대한 예측 성능에서 순위를 매겨 최종적으로 10개의 Feature를 선정하고, 실제 하드웨어에서 연산을 수행합니다. (g) 단계에서 실제 성능과 연산 가능 유무를 확인하여 (a), (c)와 (f) 모델에 대하여 Online Learning을 수행합니다.

% 성능 예측 모델을 통해 Latency가 가장 낮을 것으로 예측되는 파라미터를 탐색합니다. 탐색된 파라미터를 `Top Candidates`라 하며, 예측한 성능이 실제 보드에서 연산함으로 써, `Cost Model`에 대하여 점진적으로 `Profiling`하여 하나의 레이어에 대하여 최적의 하이퍼 파라미터를 탐색합니다.

\subsubsection{탐색 Search Space와 Feature 정의}

% 새롭게 정의되는 파라미터들에 대한 소개
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{Joobin/TEMP-Figure/Feature.png}
  \caption{The Overview}
  \label{fig:overview}
\end{figure}

프로파일링 과정에서 얻을 수 있는 feature(파라미터)는 Feature와 Hidden-Feature 이다. Feature는 프로파일링 실행 입력으로 주는 파라미터로 convolution 연산 구성과 커널 구성이 해당된다. 한 convolution에 대해서 최적화하기 때문에 convolution 연산 구성은 고정적이고, 커널 구성은 가변적이다. Hidden-Feature는 가변적인 Feature 값에 따라 고정되는 내부 연산 값을 의미하며, 커널 연산 과정에서 loop의 횟수나 특정 변수의 값 등에 해당된다. 가변적인 Feature와 Hidden-Feature가 이후 튜닝과정의 입력으로 사용된다.
Random Feature는 레이어 정보에 대한 Feature와 함께, 고정적인 값으로는 Convolution 연산 구성과 가변적인 것은 커널 구성이 해당 된다.  프로파일링은 neural network 연산 형태에 따른 HW 실행 코드를 자동으로 생성을 하여 입력 파라미터에 대한 실행 결과를 얻는 과정이다. neural network 연산에 영향을 주는 파라미터의 모든 search space 탐색한다. 일부 파라미터는 실행되지 않거나 기댓 값과 결과가 다를 수 있어 검증 과정이 필요하다. (피처는 설정할 수있는 값 + 내부적으로 연산등으로 얻을 수 있는 값 2가지로 존재) 얻은 피처들을 활용하여 xgboost 모델을 온라인 러닝을 진행한다.(진행과정 더 자세히)
한 모델에 대해서, EVTA에서 실행되는 연산 중에 동일한 연산을 제외하고 프로파일링 진행한다. ResNet18의 경우 총 10개의 convolution에 대해서 프로파일링을 진행한다. 위 표에서 H/W/C는  height와 width, channel을 의미하며, KH/KW/KC는 커널의 height와 width, channel을 의미한다. P는 padding size, S는 stride size, OH/OW는 output height와 output width를 의미한다.

\subsection{Hidden Parameter Extractor}

컴파일러가 코드 생성하는 과정에서 하드웨어에서 실제로 몇 번의 연산이 수행되는지 분석하여 새로운 Feature를 추출합니다. 추출된 정보는 Micro Kernel 구성이나 레이어 구조의 변동에 따라 달라질 수 있는 가변적 요소도 포함이되어 있으며, 암묵적인 최적화의 파라미터의 값일 수 있습니다. 외부에서 변동되는 파라미터의 값은 미미하지만 내부 Hidden Feature에 대한 변화는 상이할 수 있거나 그 반대가 존재할 수 있다. 대표적으로 보드마다 상이하지만, EVTA의 경우에는 Hidden Feature의 값은 ~\ref{tab:commands}가 존재하였다. 타겟 딥 러닝 컴파일러에 맞춰서 Hidden Parameter 를 추출하여 기존에 레이어나 커널의 Knobs의 값을 활용하던 것을 컴파일러 부터 생성된 Feature를 함께 학습하여 타겟 하드웨어 대한 Feature 관계성과 구조를 빠르게 학습하는 것에 기여한다.

\subsection{Auto-Tuning}

최적의 HyperParameter 탐색, 하이퍼 파라미터의 유효 검증, 유효한 하이퍼 파라미터의 예상되는 레이턴시 예측 모델로 3개로 구성이 되어있다. 본 연구에서 사용된 예측 모델은 추가적인 데이터를 통해 점진적으로 학습하기 위해 Online Learning 학습이 가능한 XGBoost~\cite{xgboost}와 기법은 model-data 갱신 기법을 사용하였다. 학습하는 과정은 아래와 같다. (1) 초기에 아무 지식 없는 상황에서 예측을 하게 된다면 초기에 방향성을 잘못 잡거나 초기 학습 상태에 대하여 많은 영향이 끼치므로, Online Learning을 수행하기 전에 충분한 Latency 정보를 수집하도록 한다. (2) 초기에 Valid나 Invalid한 값을 포함하여 실제 하드웨어에서 50회 연산을 수행하였을 때 충분한 데이터의 수집이 되었다고 판단하여 학습을 수행한다. (3) 그 이후로 5개의 데이터가 생성이 될 때마다 Online Learning을 수행하도록 한다. (4) Predict Best Feature, Predict Latency 그리고 Hyper Parameter Validation는 실제 하드웨어에서 유효한 값만을 활용하여 학습에 활용한다. (5) 최종적인 하이퍼 파라미터를 3개의 신경망 모델에 대하여 갱신하도록 한다. 이때, Out of Distribution[논문]관련하여 예측을 수행할 때 유효하지 않은 값을 함께 활용하여 학습에 사용한다면 오류 데이터에 대한 학습 양이 많아 편향적인 학습 결과가 나게 되는 사례가 많다. 따라서 학습은 정상 데이터만을 활용하여 학습하고, 정상적인 데이터만을 예측하도록 만들고 또한 데이터간의 관계성을 예측하도록 학습한다. 

\textbf{Predict Best Feature}는 Latency가 낮을 것으로 예상이 되는 Micro Kernel에 연산, 타일링의 하이퍼 파라미터를 탐색한다. 이 과정에서는 값이 유효한지 유효하지 않는지에 대한 검사를 수행하지 않고, 오직 내부적인 하이퍼 파라미터의 중요성에 초점을 통해 최대한의 최선의 하이퍼 파라미터를 탐색하도록 한다.  

Predict Candidates(for Generate Hyper Parameter)는 하이퍼 파라미터를 예측하기 위해서 내부 파라미터에 대하여 예측하기 위해 Rank와 Regress, 2가지로 실험을 진행하였다. Rank는 순서나 우선순위를 예측하는 데 특호돠이 있으며 주로 검색 엔진에서 문서의 순위를 매기거나 추천 시스템에서 항목의 선호도를 예측하는 데 활용된다. 랭킹 문제에서 XGBoost는 순위 손실 함수(Rank Loss Function)를 사용하여 학습한다. 랭킹 모델은 주로 쌍(pairwise) 비교에 기반한 손실 함수를 사용하여 순서에 민감한 최적화를 수행합니다. 이 과정에서는 두 항목 간의 순위 차이가 예측 목표가 되며, 순위가 올바르게 예측되도록 하는 방향으로 모델이 학습한다. 이를 통해 하이퍼 파라미터에 대한 순위에 대하여 최적화하는 방향으로 학습한다. Regress는 연속적인 수치를 예측하는 데 사용되는 회귀 모델이, 하이퍼 파라미터로 인한 변화량이 선형적인 경우 주로 활용된다. 손실 함수는 Mean Squared Error(MSE)를 활용하여 각 데이터 포인트의 실제 값과 예측 값 간의 차이를 최소화하는 것을 목적으로 한다. 이를 통해 연속적인 하이퍼 파라미터에서 출력 값을 정확하게 예측한다.


\textbf{Hyper Parameter Validation}은 모델은 먼저 Predict Best Feature로부터 생성된 하이퍼 파라미터가 실제 하드웨어에서 연산하였을 때 유효하게 연산이 수행가능한지 검증한다. Predict Best Feature에서 하이퍼 파라미터를 생성하고, 생성된 하이퍼 파라미터를 Hyper Parameter Validation 과정을 통해 Valid한 값이 20개가 생성이 되도록 계속하여 생성을 한다. 그리고 생성된 20개의 하이퍼 파라미터를 실제로 컴파일러를 통해 컴파일을 수행하여 내부에 숨겨진 추가적인 Feature를 Extract하는 과정을 수행한다.

\textbf{Predict Latency}는 하이퍼 파라미터와 내부 하이퍼 파라미터로 구성된 20개의 세트 데이터들이 예상되는 Latency를 예상한다. 레이턴시가 예측된 20개의 하이퍼 파라미터들은 레이턴시를 기준으로 정렬하여 상위 10개의 데이터만 실제 하드웨어에서 연산을 수행하여 하이퍼 파라미터와 레이턴시를 프로파일링하여 보정한다. 이 과정에서 실제 하드웨어에서 연산이 되지 않는다면 해당 데이터는 버리고 남은 데이터만 활용하여 학습에 활용하도록 학습 데이터셋에 추가한다. 따라서 하이퍼 파라미터를 기준으로 컴파일을 수행하는것은 1회 사이클마다 20번을 수행하고, 실제 하드웨어에서 연산을 수행하는 것은 10개만이 수행된다. 그렇기 때문에 Evaluation결과에서 그래프의 변화는 실제 하드웨어에서 연산하는 횟수로 표현이 되므로 Epoch 는 10씩 증가하고 Latency 또한 Epoch의 10 단위로 감소하는 것을 확인 할 수 있다.



% 하이퍼 파라미터에 대한 Valid 검사에 대한 내용
% TODO: 만약에 이 곳에 쓸만한 내용이라면, EVTA와 NMP, ACL 간 예외 처리에 대한 내용 및 컴파일 에러가 가능한 가능성 퍼센트 출력
% 너무 자세하다... 조금 더 러프하고 설득력을 가져가자.

% Contribution 내용 : 

% - Validate Hyper Parameter based on Machine Learning
% - Exploit Hidden Feature from Generated Code
% - 향상된 하이퍼 파라미터 탐색 능력

% Figure 그림 내용 설명

% 본 논문에서는 기존의 라이브러리에서 활용할 수 있는 데이터들을 사용하여 최적화를 진행하고자 한다.

% 위 그림은 실험 흐름에 대해 나타내는 것이다. tensorflow나 pytorch와 같은 라이브러리에서 만든 모델 혹은 ~인공지능 모델을 다양한 하드웨어에서 실행시키기 위해서는 각 하드웨어에 맞는 컴파일러 라이브러리가 필요하다. 이런 컴파일러 라이브러리는 자주 쓰이는 특정한 연산에 대해서만 최적화되어있다. 기존 연구에서는 이를 기존에 이미 만들어진 라이브러리는 최적화를 위해 필요한 코드는 블랙박스기 때문에 새로운 라이브러리를 만들어서 연구가 진행되었다. 이는 기존에 만든 라이브러리를 활용할 수 없기 때문에 많은 비용과 시간이 드는 방법이다. 이를 개선하기 위해서 기존의 컴파일러 라이브러리에서 활용할 수 있는 데이터를 가지고 최적화하는 방법을 제안한다. (자세한 방법 적기)
% 해당 과정은 크게 프로파일링 과정과 튜닝 과정으로 나눌 수 있다.






==> Paper/05_algorithm_graphivz.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{Paper/Resources/3Stage_v2.png}
    \caption{Flow Autotuing by NesTuner}
    \label{fig:flow_of_nestuner}
\end{figure}

% digraph G {
%     // 전체 그래프 속성
%     graph [splines=ortho]
    
%     rankdir=LR  // 왼쪽에서 오른쪽으로 흐름 설정
    
%     node [fontsize=10]
    
    
%     // 주요 노드 정의
%     neural_network [label="Neural Network", shape=ellipse, style=filled, color=lightblue]
%     extract_neural_network [label="Task Extraction", shape=box, style=filled, color=lightgrey]
%     extract_feature_in_task [label="Feature Extraction", shape=box, style=filled, color=lightgrey]

%     // NesTuner 클러스터 정의
%     subgraph cluster_1 {
%         // edge [len=4f, fontsize=5]
%         label = "NesTuner"
%         style=filled
%         color=lightyellow
%         fontsize=15
        
%         // 클러스터 내부 노드 정의
%         entry [label="Start", shape=box, style=filled, color=white]
        
%         model1 [label="Generate Random or Predict", shape=component, style=filled, color=white]
%         model2 [label="Validate", shape=component, style=filled, color=white]
%         model3 [label="Predict w/ Hidden Features", shape=component, style=filled, color=white]
%         compiler [label="Compile", shape=component, style=filled, color=white]
%         profiling [label="HW Profiling", shape=box, style=filled, color=white]
%         update [label="Update Model", shape=box, style=filled, color=white]
%         exit [label="Next Step?", shape=diamond, style=filled, color=white]
        
%         // NesTuner 클러스터 내부 흐름
%         entry -> model1 [label="(2) Layer & Kernel"]
%         entry -> model3 [label="Layer & Kernel"]
%         model1 -> model2 [label="(3) Candidates"]
%         model2 -> model1 [label="(4) if Fail/Re Candidate", style=dashed]
%         model2 -> compiler [label="(5) Candidates"]
        
%         compiler -> model3 [label="Hidden Features"]
%         model3 -> profiling [label="Program"]
%         profiling -> update [label="Execution Feedback"]
    
%         update -> exit
%     }

%     // 외부 노드 정의
%     fin [label="Has Next Task?", shape=diamond, style=filled, color=lightpink]
%     real_fin [label="Outperformance Model Result", shape=box, style=filled, color=lightgreen]

%     // 주요 흐름
%     neural_network -> extract_neural_network
%     extract_neural_network -> extract_feature_in_task [label="Input: Task[]"]
%     extract_feature_in_task -> entry [label="(1) Layer, Kernel and Tiling"]


%     // 모델 업데이트 후 다음 단계
    
%     exit -> entry [label="Search Space"]
%     exit -> fin
%     fin -> extract_feature_in_task
%     fin -> real_fin [label="Output"]
% }


==> Paper/XX_Instruction.tex <==

\newpage

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

